Reasoning about Emergence of Collective Memory

We offer a very simple model of how collective memory may form. Agents keep signalling within neighbourhoods, and depending on how many support each signal, some signals "win" in that neighbourhood. By agents interacting between different neighbourhoods, 'influence' spreads and sometimes, a collective signal emerges. We propose a logic in which we can reason about such emergence of memory and present preliminary technical results on the logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{269}
\providecommand{\publicationstatus}{J. Y. Halpern and A. Perea (Eds.): Theoretical Aspects \\
of Rationality and Knowledge 2021 (TARK 2021) \\
EPTCS 335, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.335.26}{10.4204/EPTCS.335.26}}

